GNN-MultiFix: Addressing the pitfalls for GNNs for multi-label node classification

Graph neural networks (GNNs) have emerged as powerful models for learning representations of graph data showing state of the art results in various tasks. Nevertheless, the superiority of these methods is usually supported by either evaluating their performance on small subset of benchmark datasets or by reasoning about their expressive power in terms of certain graph isomorphism tests. In this paper we critically analyse both these aspects through a transductive setting for the task of node classification. First, we delve deeper into the case of multi-label node classification which offers a more realistic scenario and has been ignored in most of the related works. Through analysing the training dynamics for GNN methods we highlight the failure of GNNs to learn over multi-label graph datasets even for the case of abundant training data. Second, we show that specifically for transductive node classification, even the most expressive GNN may fail to learn in absence of node attributes and without using explicit label information as input. To overcome this deficit, we propose a straightforward approach, referred to as GNN-MultiFix, that integrates the feature, label, and positional information of a node. GNN-MultiFix demonstrates significant improvement across all the multi-label datasets. We release our code at https://anonymous.4open.science/r/Graph-MultiFix-4121.

==> additionalanalysis.tex <==
\subsection{Additional analysis of \mymodel}
 The experiments are designed to answer the following research questions: (i) Does different modules in \mymodel provide useful information for the node classification task?


\subsubsection{Modules In \mymodel}
\label{app:modules}
To answer the first question of the information provided by the positional embeddings, we load \mymodellin trained on one split of the \blog dataset and visualize the learned weights $\mathbf{W}$ in the last fusion layer using heatmap in Figure \ref{fig:weights_all}. As all non-linearity is removed in \mymodellin, the learned weights can be seen as the importance assigned by the model to the different parts of our model, we visualize the weights for feature representation in Subfigure \ref{fig:weights_fp}, label representation in Subfigure \ref{fig:weights_lp}, and positional representation in Subfigure \ref{fig:weights_pe}.


Since we concatenate $\mathbf{h}^{(K)}_{f_v} \in \mathbb{R}^{n \times \text{hidden\_dim}}$, $\mathbf{h}^{(N)}_{l_v} \in \mathbb{R}^{n \times C}$, and $\mathbf{\phi}_v \in \mathbb{R}^{n \times \text{PE\_dim}}$ as the input of the fusion layer, we denote $H = \text{hidden\_dim} + C + \text{PE\_dim}$, thus $\mathbf{W} \in \mathbb{R}^{C \times H}$ and the weights learned for feature representation, label representation, and positional representation have the shape of $\mathbf{W}_{f_v} \in \mathbb{R}^{C \times \text{hidden\_dim}}$, $\mathbf{W}_{l_v} \in \mathbb{R}^{C \times C}$, and $\mathbf{W}_{\phi_v} \in \mathbb{R}^{C \times \text{PE\_dim}}$ respectively. 


In our visualization, the darker the cell is, the higher the weights are. However, small negative weights learned by the model can also be meaningful, indicating negative correlations between the input and output. Thus, the more contrastive the weights are, the more important are the part of the input for the output. 

% As shown in Figure \ref{fig:weights_visualization}, in the dataset without input features, our model learns to focus on the positional embedding to break the graph isomorphism and generate different embeddings for similar nodes, thus enhance the expression ability of graph neural networks.


\begin{figure}[!h]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figs/linear_weights_all.png}
        \caption{Visualization of weights in the fusion layer of our linear model on \blog.}
        \label{fig:weights_all}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figs/linear_weights_fp.png}
        \caption{Visualization of weights in the linear model for feature propagation on \blog.}
        \label{fig:weights_fp}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figs/linear_weights_lp.png}
        \caption{Visualization of weights in the linear model for label propagation on \blog.}
        \label{fig:weights_lp}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figs/linear_weights_pe.png}
        \caption{Visualization of weights in the linear model for positional representation on \blog.}
        \label{fig:weights_pe}
    \end{subfigure}
    \caption{Visualization of weights in the fusion layer of \mymodellin trained on \blog dataset. All the subplots use the same value bar as in \ref{fig:weights_pe}.}
    \label{fig:weights_visualization}
\end{figure}

\begin{figure}[!h]
    
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\textwidth]{figs/lineplot_losses_linear_blogcatalog.png}
        \caption{\mymodellin on the \blog dataset.}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.47\textwidth}
        \includegraphics[width=\textwidth]{figs/lineplot_losses_linear_dblp.png}
        \caption{\mymodellin on the \dblp dataset.}
    \end{subfigure}
    \caption{Visualization of the training loss of \mymodellin on the \blog and \dblp dataset. Captions of the subfigure marks the name of the model and the dataset. }
    \label{fig:train_dym}
\end{figure}




\subsubsection{Homophily Recovery}
\label{app:recover_homo}
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-50pt} 
  \begin{center}
    \includegraphics[width=0.4\textwidth]{figs/homophily.png}
  \end{center}
  \caption{The label homophily predicted for \homolevel by \mymodelMlp and the true label homophily.}
  \label{fig:homophily}
  \vspace{-20pt}
\end{wrapfigure}

We use \mymodelMlp trained for the varying homophily experiment on the five synthetic datasets with varying label homophily. We use $0.5$ as a threshold to convert the output probabilities of our model into predictions and calculate the label homophily of the predicted graph. The label homophily levels of the predicted graph and the original graph are summarized in the Figure \ref{fig:homophily}. As shown in the figure, our model successfully recovers the label homophily in the input graph.

==> modelTikz.tex <==

\begin{tikzpicture}[
    node distance=1.5cm and 2.5cm,
    rounded corners,
    thick,
    every node/.style={align=center},
    block/.style={draw, minimum width=2cm, minimum height=1.2cm, text centered, fill=green!30, text width=2.5cm},
    labelblock/.style={draw, minimum width=2cm, minimum height=1.2cm, text centered, fill=blue!20, text width=2.5cm},
    positionblock/.style={draw, minimum width=2cm, minimum height=1.2cm, text centered, fill=purple!20, text width=2.5cm},
    mlp/.style={draw, minimum width=2cm, minimum height=1.2cm, text centered, fill=green!50, text width=2cm},
    arr/.style={->, thick}
]

% Graph representation G(V,E)
\node (graph) [block, fill=green!30] {Graph\\ $\mathcal{G} = (\mathcal{V}, \mathcal{E})$};

% Feature representation layers
\node (feature1) [block, right=of graph] {Layer k};
\node (feature2) [block, right=of feature1] {Layer k+1};
\node (featuretext) [above=0.5cm of feature1] {Feature Representation};

% Label representation layers
\node (label1) [labelblock, below=1cm of feature1] {Layer n};
\node (label2) [labelblock, right=of label1] {Layer n+1};
\node (labeltext) [above=0.5cm of label1] {Label Representation};

% Positional representation
\node (pos1) [positionblock, below=1cm of label1] {};
\node (postext) [above=0.5cm of pos1] {Positional Representation};

% Hf, Hl, Hv
\node (h_f) [block, right=of feature2, fill=orange!50, text width=1.5cm] {$h^{(K)}_{f_v}$};
\node (h_l) [block, below=0.5cm of h_f, fill=blue!50, text width=1.5cm] {$h^{(N)}_{l_v}$};
\node (h_v) [block, below=0.5cm of h_l, fill=purple!50, text width=1.5cm] {$\Phi_v$};

% Concatenated vector h_v
\node (concat) [block, right=of h_v, fill=green!50, text width=2cm] {$h_v$};

% MLP
\node (mlp) [mlp, right=of concat] {MLP};
\node (y_hat) [mlp, right=of mlp] {$\hat{Y}_v$};

% Arrows
\draw[arr] (graph) -- (feature1);
\draw[arr] (feature1) -- (feature2);
\draw[arr] (graph) -- (label1);
\draw[arr] (label1) -- (label2);
\draw[arr] (graph) -- (pos1);
\draw[arr] (feature2) -- (h_f);
\draw[arr] (label2) -- (h_l);
\draw[arr] (pos1) -- (h_v);
\draw[arr] (h_f) -- (concat);
\draw[arr] (h_l) -- (concat);
\draw[arr] (h_v) -- (concat);
\draw[arr] (concat) -- (mlp);
\draw[arr] (mlp) -- (y_hat);

\end{tikzpicture}


